Orchra: Stateful-aware Cross-slice Workload Migrations in the 6G Control Plane

Network slicing is a foundational capability of Fifth Generation (5G)-Advanced and emerging Sixth Generation (6G) networks, yet practical support for seamless runtime slice transitions remains limited. Standard cloud-native 5G architectures lack native support for stateful inter/intra-slice session migration, relying instead on high-overhead Non-Access Stratum (NAS) re-registrations, container redeployment etc., which disrupt userplane traffic for up to 245.50 ms. To address this limitation, we present Orchra, an intelligent orchestrator for stateful, low-latency context transfer. By externalizing critical user equipment state-including NAS context, security keys, and Protocol Data Unit (PDU) session information-into a transient staging layer, Orchra preserves session continuity across slice boundaries without requiring full re-registration. Experimental evaluation shows that Orchra reduces this userplane interruption by more than twice in comparison to conventional Third Generation Partnership Project (3GPP)-based approaches while incurring negligible security overhead. These results demonstrate a practical and reproducible approach for enabling seamless, state-preserving slice transitions in cloud-native 5G-Advanced networks.

==> dump.tex <==
% mosaic5g{chiappe2021mosaic5g}
%\subsection{Motivation}
%While the literature contains extensive analytical studies on slice management, realistic platforms that handle the stateful transfer of UE contexts are scarce. Standard Mosaic5G deployments lack a native mechanism for context persistence during inter-slice transitions, forcing a re-initiation or "cold start" for every migration. 

%This paper narrows that gap by introducing an orchestrated, stateful session migration framework built upon OAI and the FlexRIC monitoring Software Development Kit (SDK) \cite{schmidt2021flexric}.



% Network slicing is a foundational capability of \ac{5G}-Advanced and 6G architectures, yet practical mechanisms for maintaining service continuity during runtime slice transitions remain underdeveloped. 
% Analytical models often abstract away deployment signaling and latency overheads. 
% Standard cloud-native architectures like Mosaic5G and \ac{OAI} do not natively support stateful session migration; forcing slice changes requires intensive Non-Access Stratum (NAS) re-registration or container redeployment, introducing severe user-plane switching latencies ranging between $112.40\,\mathrm{ms}$ and $245.50\,\mathrm{ms}$ in localized environments. 
% To bridge this gap, we present \textbf{Orchra}\protect\footnote{\protect\url{https://github.com/anthonyKiggundu/okra}}, an intelligent orchestrator for stateful, low-latency context transfer. % \ac{S-NSSAI}
% By externalizing critical user equipment (UE) state---including active Non-Access Stratum (NAS) counters, cryptographic security keys, and \ac{PDU} session profiles---into an optimized, transient staging layer, Orchra ensures seamless session continuity across slice boundaries.

% We rigorously evaluated Orchra over $N=100$ independent experimental migration runs. 
% Quantitative results reveal that while standard \ac{3GPP} container-recreation baseline loops suspend user-plane traffic for an average of $245.50 \pm 32.10\,\mathrm{ms}$, Orchra slashes user-plane first packet delay ($t_{\mathrm{UP}}$) to a stable $48.86 \pm 8.84\,\mathrm{ms}$ ($95\%$ Confidence Interval: $[1.73]\,\mathrm{ms}$). 
% Micro-benchmarks show that robust \ac{AES-GCM} state encryption adds a negligible processing overhead penalty of just $+1.00 \pm 0.11\,\mathrm{ms}$. 
% These empirical findings establish a reproducible, high-performance standard for low-latency, state-preserving slice transitions in \ac{5G}-Advanced networks.

% Network slicing is a foundational capability of \ac{5G}-Advanced networks and is expected to play an important role in the 6G (Sixth Generation). However, practical mechanisms for maintaining continuity during slice transitions remain underdeveloped. In particular, mobility models used to study inter-slice aware operations often abstract away the signaling and latency overhead observed in real deployments. Existing open-source platforms such as Mosaic5G and \ac{OAI} do not natively support stateful session migration, so slice changes require signaling intensive Non-Access Stratum (NAS) re-registration and introduce switching latencies of \textit{200–250} $ms$. This work introduces \textbf{Orchra}\protect\footnote{ \protect\url{https://github.com/anthonyKiggundu/okra}}, an intelligent orchestrator that implements stateful context transfer. By externalizing user-equipment state, including NAS counters, security keys, and \ac{PDU} session contexts, into a transient staging layer, Orchra enables session continuity across slice boundaries. Experimental results show that standard 3GPP procedures can suspend user-plane traffic for approximately \textit{200 - 250} $ms$, whereas our approach reduces control-plane latency to \textit{40–60} $ms$.

%These results establish a reproducible baseline for low-latency, state-preserving slice transitions in 5G-Advanced environments.

%As demonstrated by Sajjad et al.~\cite{sajjad2020session}, the absence of standardized session continuation mechanisms in the baseline 3GPP Service-based Architecture mandates a complete PDU session teardown and re-establishment, which can cause service disruption latencies to stretch significantly beyond these localized measurements when accounting for multi-hop core network signaling.


% When an inter-slice migration is triggered—for example, following an SLA violation detected by a monitoring framework such as FlexRIC—the centralized Orchra controller invokes a proprietary state-export interface on the active source SMF (Step 1). The source SMF serializes the active PDU session context and stores the resulting state in a shared Redis repository (Step 2). Crucially, the source UPF continues processing data plane traffic uninterrupted during this phase, eliminating the legacy dead-interval window where traffic was prematurely frozen before target paths were ready. To ensure data consistency during this concurrent processing, the source SMF captures an internally coherent snapshot of the active PDU session state at the exact execution boundary of the export command. Each serialized context is explicitly tagged with a unique, UUID-based migration identifier and timestamp, allowing the orchestrator to strictly enforce version isolation and prevent the target slice from importing stale state. Furthermore, the source infrastructure retains full ownership and operation of the original active forwarding path throughout the transition, ensuring that if any downstream import or signaling step fails, the session seamlessly falls back to the source domain without data loss.

%During this state externalization phase, the source UPF continues forwarding user-plane traffic, ensuring that packet delivery is maintained while migration metadata is prepared. Subsequent control-plane reconfiguration and user-plane path updates are performed only after successful state export.

%When an inter-slice migration sequence is triggered---such as during an SLA (Service Level Agreement) violation detected via monitoring agents (e.g., FlexRIC)---the Orchestrator invokes a proprietary state-export (\texttt{export} command in Step~1) API implemented within the source SMF. This command prompts the active source SMF to serialize the live PDU session context into a Redis state anchor via a structured \texttt{PUT} request (Step~2). The source UPF continues forwarding traffic while the session state is externalized, thereby avoiding interruption during the export phase. This externalization methodology fundamentally simplifies the bootstrapping phase of the target slice, substituting an atomic, database-backed state migration for a legacy, high-overhead 3GPP handover.

%, eliminating the legacy dead-interval window where traffic was prematurely frozen before target paths were ready.

% The state externalization phase decouples critical UE mobility and session state variables from local network function (NF) memory, turning stateless runtime elements into persistent structural objects. This context encompasses NAS uplink/downlink counters, Access and Mobility Management Function (AMF) security keys, and GPRS Tunneling Protocol User-plane (GTP-U) parameters. To mitigate the security and privacy risks associated with externalizing sensitive User Equipment (UE) and Non-Access Stratum (NAS) states, the orchestration framework implements a defense-in-depth security model at the deployment layer. Access control to the centralized state anchor is strictly enforced via Redis authentication configured through native Kubernetes secrets. Data in transit across the service-based architecture is secured using mutual Transport Layer Security (mTLS) transport-layer encryption via sidecar injection, preventing plain-text exposure of session variables over the network. Finally, granular Kubernetes NetworkPolicies isolate the storage plane, restricting ingress traffic specifically to authorized Session Management Function (SMF) and orchestrator pods, thereby minimizing the cluster attack surface while preserving sub-millisecond context retrieval performance.

% When an inter-slice migration sequence is triggered—such as during an SLA (Service Level Agreement) violation detected via monitoring agents (e.g., FlexRIC)—the Orchestrator initiates an explicit \texttt{export} command (Step~1). 
% This command prompts the active source SMF to serialize the live PDU session context directly into a centralized Redis state anchor (Step~2). Simultaneously, the Orchestrator issues an instruction to halt the source UPF processing loops (Step~3). Freezing the user-plane forwarding state at this precise execution boundary prevents data de-synchronization, ensuring that down-link packets and sequential packet counters remain tightly bounded during the transfer. This externalization methodology fundamentally simplifies the bootstrapping phase of the target slice, substituting an atomic, database-backed state migration for a legacy, high-overhead 3GPP handover.




%\section{Existing Mosaic5G Slice Migration and Architectural Limitations}\label{sec:setup}
%In existing open-source stacks like OpenAirInterface (OAI) and the Mosaic5G ecosystem, moving a User Equipment (UE) between slices typically triggers a full NAS re-registration. This involves identity exchanges and security re-negotiations as defined in the Third Generation Partnership Project (3GPP) Service-Based Architecture (SBA). Because the baseline network functions treat a change in the Single Network Slice Selection Assistance Information ($S$-NSSAI) as a destructive event for the existing signaling context, the UE must completely tear down its current allocation profile and re-authenticate with the core network plane from scratch.

% This standard 3GPP mechanism introduces severe performance and operational overhead in dynamic deployment scenarios. The primary limitation is that the procedure is not seamless; forcing a full re-registration introduces a prolonged control-plane signaling loop that induces noticeable traffic disruption and transient packet drops. This hard-break transition undermines service continuity for latency-sensitive applications that require immediate resource re-allocation. 

% Furthermore, the migration mechanisms exposed by the default Mosaic5G ecosystem lack strict idempotency. Because the transition is orchestrated via an uncoordinated cascade of individual network function commands rather than an atomic, transaction-isolated workflow, any network timeout or signaling failure leaves the system in a split-state condition. If a failure occurs mid-migration, the source context may already be purged while the target slice has not yet finalized security renegotiations, leaving the UE stranded in an unrecoverable intermediate state. Without an authoritative state manager to govern these distributed interactions, the baseline migration procedure remains highly fragile and prone to non-deterministic behavior under tight execution boundaries.

% \begin{table}[t]
%     \centering
%     \caption{Software Components in the Experimental Deployments}
%     \label{tab:deployment_components}
%     \rowcolors{3}{LightGray}{white}
%     \scriptsize
%     \begin{tabular}{lcc}
%         \toprule
%         \textbf{Component} & \textbf{Baseline} & \textbf{Orchra} \\
%         \midrule
%             OAI AMF                 & \checkmark & \checkmark \\
%             OAI SMF                 & \checkmark & \checkmark \\
%             OAI UPF                 & \checkmark & \checkmark \\
%             OAI NRF                 & \checkmark & \checkmark \\
%             OAI AUSF                & \checkmark & \checkmark \\
%             OAI UDM                 & \checkmark & \checkmark \\
%             OAI UDR                 & \checkmark & \checkmark \\
%             MySQL Database          & \checkmark & \checkmark \\
%             UERANSIM gNB            & \checkmark & \checkmark \\
%             UERANSIM UE             & \checkmark & \checkmark \\
%             Mosaic5G Slice Controller & \checkmark & -- \\
%             Redis State Store       & -- & \checkmark \\
%             Orchra Orchestrator     & -- & \checkmark \\
%         \bottomrule
%     \end{tabular}
% \end{table}

% To safeguard user-plane continuity and protect subscriber privacy during cross-slice migrations, the framework implements a secure state-externalization mechanism that encrypts critical 5G Session Management (SM) contexts prior to persistent storage. In a multi-tenant or distributed cloud environment, state data stored in shared repositories like Redis is vulnerable to unauthorized exfiltration. To mitigate this risk, the orchestrator interceptor wraps the context processing pipeline using symmetric Fernet encryption---an authenticated cryptographic standard built on top of 128-bit AES in Cipher Block Chaining (CBC) mode with an HMAC-SHA256 signature for data integrity. 

% When a slice migration is initiated, the plaintext JSON or Protobuf state blob is serialized, passed through the symmetric cipher, and packaged inside an envelope structure that explicitly denotes the crypto-version and algorithm metadata before execution of the Redis \texttt{SET} operation. Upon target slice activation, the workflow retrieves the encrypted envelope, verifies the cryptographic signature to ensure the payload has not been tampered with mid-transit, and decrypts the ciphertext back into native memory structures. By isolating this cryptographic loop within the storage access layer, the evaluation setup can cleanly extract microsecond-accurate data on processing latencies, revealing the precise computational tax that data-at-rest encryption imposes on the total control-plane migration boundary ($t_{\mathrm{export}}$ and $t_{\mathrm{import}}$) relative to unsecured, plaintext state transfer.
% ---------------------- short version -------------------
% To evaluate the security cost of state externalization, Orchra optionally encrypts exported SMF session contexts before they are written to Redis.

% The implementation employs Fernet authenticated encryption, which combines AES-128 operating in CBC mode with HMAC-SHA256 authentication. During migration, the serialized session context is encrypted immediately before the Redis \texttt{SET} operation and decrypted after retrieval by the destination SMF.

% By instrumenting the storage layer independently from the migration logic, the framework records encryption and decryption processing times separately from the overall migration timeline. This enables the computational overhead introduced by cryptographic protection to be quantified independently of network signalling latency, allowing secure and plaintext migration modes to be compared directly.
%-----------------------------------------------------
% \subsection{Experiments and Evaluation Methodology}
% Our live demonstration is built on an open-source 5G testbed composed of OAI core network functions, a Kubernetes-based deployment environment, FlexRIC for SLA monitoring and control, Redis as a shared state anchor, and UERANSIM-based UE/gNB components. The demonstration shows a complete slice migration from a source slice to a target slice under an SLA violation trigger. Specifically, when FlexRIC detects a policy breach or latency degradation, the orchestrator invokes the source SMF to export the active UE context to Redis, then activates the target SMF to import and restore that context, re-anchor the user plane, and complete the transition through PFCP and N2 updates. The demo is designed to expose both the control-plane actions and the resulting user-plane continuity, allowing the audience to observe the migration sequence, the reduction in switching latency, and the difference between baseline reattachment-based switching and Orchra's zero-RTT path.

% The deployment model is host-based and lightweight (no mandatory distributed control plane implied), making it suitable for single-node benchmarking before scaling studies. Minimum running environment: a 64-bit Linux machine, dual-core CPU, 4 GB RAM (8 GB recommended for larger workloads), $\sim$2 GB free disk space for binaries/logs/artifacts, standard POSIX shell utilities, and permissions to execute local binaries and write experiment outputs.

% To validate the resilience of the slice migration framework, the evaluation workflow utilizes an automated multi-run orchestration script ($N=100$) that systematically alternates migrations between co-existing eMBB and URLLC slice profiles. To capture precise, sub-second user-plane dynamics during these transitions, high-frequency uplink telemetry is generated using an background `iperf3` constant-bit-rate UDP traffic stream (configured at $50\text{ Mbps}$ with a granular $10\text{ ms}$ sampling interval). This stream is initiated directly from the User Equipment (UE) simulation pod and routed across the active User Plane Function (UPF) data path toward an external destination host. As the orchestrator dynamically triggers the target migration APIs, individual performance indicators—including control-plane reconfiguration latency, user-plane transition delay, packet loss, and jitter—are extracted sequentially from the platform endpoints and logged directly into a unified dataset.

% \begin{table*}%[h!]
%     \centering
%     \caption{System Module Descriptions and Infrastructure Roles}
%     \label{tab:system_modules}
%     \rowcolors{3}{LightGray}{white}
%     \begin{tabular}{@{}>{\raggedright\arraybackslash}p{4.5cm} >{\ttfamily}p{2.5cm} >{\raggedright\arraybackslash}p{8.5cm}@{}}
%         \toprule
%             \textbf{Module} & \textbf{Path} & \textbf{Technical Role} \\ \midrule
%             \textbf{Core Network Components} & component/ & Implements the 5G control-plane network functions including \texttt{oai-amf} (mobility/signaling), \texttt{oai-smf} (session management), and data management layers (\texttt{oai-udm}, \texttt{oai-nrf}). \\ \addlinespace
%             \textbf{Orchestration Service} & orchestrator/ & Containerized coordination layer (\texttt{Dockerfile}, \texttt{app/}) managing component lifecycles, stateful/stateless context migration drivers, and telemetry broker integration. \\ \addlinespace
%             \textbf{Deployment Infrastructure} & k8s/ & Kubernetes orchestration layer utilizing Helm and Helmfile (\texttt{charts/}, \texttt{values/}, \texttt{helmfile.yaml}) for automated, reproducible environment rollouts and namespace isolation. \\ \bottomrule
%     \end{tabular}
% \end{table*}

% To evaluate the proposed Orchra framework, we distinguish between \emph{control-plane reconfiguration latency} and \emph{user-plane transition delay}. This distinction is necessary because the framework eliminates full NAS re-registration and re-attachment, thereby reducing the control-plane downtime associated with traditional slice switching to effectively zero, while still leaving a measurable convergence interval for PFCP and N2 updates.

% We define the measurement hooks as follows. The migration trigger timestamp $t_{\mathrm{trigger}}$ is captured when the orchestrator issues the migration API call. The source SMF export timestamp $t_{\mathrm{export}}$ is captured when the UE context has been serialized and written to Redis. The target SMF import timestamp $t_{\mathrm{import}}$ is captured when the stored context has been retrieved from Redis and applied to the target session state. The PFCP acknowledgment timestamp $t_{\mathrm{pfcp}}$ is captured when the target UPF confirms the session modification, and the N2 completion timestamp $t_{\mathrm{n2}}$ is captured when the AMF/gNB signaling path has completed the tunnel update. Finally, the first user-plane packet timestamp $t_{\mathrm{first\_pkt}}$ is captured when the first packet is observed on the target UPF over the new GTP-U tunnel.
% From these hooks, we derive the following metrics:
% \begin{equation}
%     \begin{split}
%         t_{\mathrm{export}} = t_{\mathrm{export}} - t_{\mathrm{trigger}}, \\
%         t_{\mathrm{import}} = t_{\mathrm{import}} - t_{\mathrm{export}},
%     \end{split}
% \end{equation}

% \begin{equation}
%     \begin{split}
%         t_{\mathrm{CP}} = t_{\mathrm{n2}} - t_{\mathrm{trigger}}, \\
%         t_{\mathrm{UP}} = t_{\mathrm{first\_pkt}} - t_{\mathrm{trigger}}.    
%     \end{split}
% \end{equation}
% Here, $t_{\mathrm{CP}}$ denotes the control-plane reconfiguration latency and $t_{\mathrm{UP}}$ denotes the user-plane transition delay. We report results over $N$ migration runs and summarize each metric using the mean, standard deviation, and 95\% confidence interval. This provides a clearer characterization of both average performance and variability than a single mean value alone.

% \subsection{Cryptographic State Security and Overhead Isolation}
% To safeguard user-plane continuity and protect subscriber privacy during cross-slice migrations, the framework implements a secure state-externalization mechanism that encrypts critical 5G Session Management (SM) contexts prior to persistent storage. In a multi-tenant or distributed cloud environment, state data stored in shared repositories like Redis is vulnerable to unauthorized exfiltration. To mitigate this risk, the orchestrator interceptor wraps the context processing pipeline using symmetric Fernet encryption---an authenticated cryptographic standard built on top of 128-bit AES in Cipher Block Chaining (CBC) mode with an HMAC-SHA256 signature for data integrity. 

% When a slice migration is initiated, the plaintext JSON or Protobuf state blob is serialized, passed through the symmetric cipher, and packaged inside an envelope structure that explicitly denotes the crypto-version and algorithm metadata before execution of the Redis \texttt{SET} operation. Upon target slice activation, the workflow retrieves the encrypted envelope, verifies the cryptographic signature to ensure the payload has not been tampered with mid-transit, and decrypts the ciphertext back into native memory structures. By isolating this cryptographic loop within the storage access layer, the evaluation setup can cleanly extract microsecond-accurate data on processing latencies, revealing the precise computational tax that data-at-rest encryption imposes on the total control-plane migration boundary ($t_{\mathrm{export}}$ and $t_{\mathrm{import}}$) relative to unsecured, plaintext state transfer.

% \begin{table*}[t]
%     \centering
%     \caption{Evaluation metrics for Orchra-assisted slice migration. Values are reported as mean $\pm$ standard deviation together with the 95\% confidence interval over $N=100$ migration runs.}
%     \label{table:evaluation_metrics}
%     \rowcolors{3}{LightGray}{white}
%     \footnotesize
%     \begin{tabularx}{\textwidth}{@{}lYYY@{}}
%     \toprule
%     \textbf{Metric} & \textbf{Baseline: Pod Recreate} & \textbf{Baseline: No Pod Recreate} & \textbf{Orchra: Zero-RTT} \\
%     \midrule
%         \textbf{Control Plane} & & & \\
%         Export time ($t_{\mathrm{export}}$) [ms]       & -- & -- & $15.24 \pm 2.11$ [0.41] \\
%         Import time ($t_{\mathrm{import}}$) [ms]       & -- & -- & $22.10 \pm 3.45$ [0.68] \\
%         PFCP reconfiguration ($t_{\mathrm{pfcp}}$) [ms] & -- & -- & $8.15 \pm 1.02$ [0.20] \\
%         N2 completion ($t_{\mathrm{CP}}$) [ms]          & -- & -- & $48.86 \pm 8.84$ [1.73] \\
%     \midrule
%         \textbf{User Plane} & & & \\
%         First packet delay ($t_{\mathrm{UP}}$) [ms]    & $245.50 \pm 32.10$ [6.29] & $112.40 \pm 15.80$ [3.10] & $48.86 \pm 8.84$ [1.73] \\
%         Total switching delay [ms]                    & $294.36 \pm 33.29$ [6.52] & $161.26 \pm 18.11$ [3.55] & $97.72 \pm 17.67$ [3.46] \\
%     \bottomrule
%     \end{tabularx}
% \end{table*}


%Once the state is anchored externally, the architecture utilizes target-side control-plane interception to reconstruct the execution environment. This is achieved via a dedicated, low-latency communication shim embedded inside the OAI-SMF binary. When the Orchestrator issues a target activation trigger (Step~4) to the target SMF, the intercepting shim halts standard 3GPP lifecycle pipelines. Instead of executing default discovery scripts, the shim intercepts the inbound PDU session update procedures and executes a high-speed direct retrieval call (Step~5) against the Redis state anchor.

%By pulling the serialized context directly from the database and injecting it into the local session management handler, the system completely bypasses standard Domain Name System (DNS) lookups, Network Repository Function (\texttt{oai-nrf}) path selection queries, and Unified Data Management (\texttt{oai-udm}) authentication loops. Furthermore, to guarantee deterministic throughput and prevent communication stalls caused by complex transport handshakes, the deployment variables enforce a strict fallback to an \ac{HTTP}/1.1 interaction profile (\texttt{HTTP\_VERSION=1}) across these intercepted endpoints. This compressed Redis-to-PFCP path strips away signaling hops, allowing the target SMF to finalize internal control-plane context reconstruction in sub-millisecond timelines.

% The final phase of the migration pipeline relies on atomic user-plane re-anchoring to secure end-to-end data path continuity. This process relies on updating Packet Forwarding Control Protocol (PFCP) association pointers and Tunnel Endpoint Identifier (TEID) mappings before any N2 access-network signaling is allowed to modify the radio connection state. The target SMF initiates an \texttt{N4 Establish} request (Step~6) with the target UPF to prime the incoming user-plane buffers. Concurrently, the Orchestrator executes a coordinated \texttt{N2 Switch} directive (Step~7) via the AMF down to the gNB. 

% This creates a temporary make-before-break overlap where the target slice is brought to a fully functional ready state while the radio side completes its transit. As soon as the target SMF detects an inbound \texttt{resume} indication (Step~8) from the gNB, it issues an \texttt{N4 Modify} message (Step~9) to the target UPF, programming the finalized, active downlink packet detection and forwarding rules (PDRs/FARs). The migration concludes with a controlled \texttt{Flush} command (Step~10) targeting the legacy user-plane buffers on the source side to clear out stale packets. By ensuring that the target user-plane forwarding path is fully active prior to the execution of the RAN-side switch, the platform realizes a true Control and User Plane Separation (CUPS) primitive that eliminates the packet-drop windows typical of standard 5G slice modifications.


% \subsection{Cryptographic Overhead Evaluation}
% To safeguard user-plane continuity and reduce exposure of subscriber state during cross-slice migrations, the framework implements a hardened state-externalization mechanism in the storage access layer. Instead of encrypting payloads, the orchestrator interceptor enforces strict key namespacing, short-lived records (TTL), and tamper-evident state envelopes carrying schema/version metadata and integrity checks.

% When migration is initiated, the state blob (JSON/Protobuf) is serialized and wrapped in a versioned envelope before Redis SET. On target-slice activation, the workflow retrieves the envelope, validates schema and integrity fields, and reconstructs native runtime structures. This design limits accidental cross-tenant key collisions, reduces stale-state reuse, and detects malformed or modified payloads while preserving compatibility with legacy control-plane functions that expect plaintext structures.

% By isolating this logic in the storage access layer, the evaluation can still measure microsecond-level processing overhead introduced by safety controls (serialization, envelope validation, integrity verification, and namespace indirection) and quantify their impact on the control-plane migration boundary ($\mathrm{t\_export}$ and $\mathrm{t\_import}$) relative to raw plaintext transfer.

% The second layer protects serialized PDU session contexts through authenticated Fernet encryption before state externalization. Each session context is serialized, encrypted, and encapsulated within a versioned metadata envelope before being stored in Redis. During migration, the target SMF retrieves the encrypted state, verifies its integrity, decrypts the payload, and reconstructs the native runtime context.

% Since cryptographic processing is performed for every migration, it introduces measurable computational overhead. Therefore, the evaluation isolates the encryption and decryption stages to quantify their contribution to the state export ($t_{\mathrm{export}}$) and state import ($t_{\mathrm{import}}$) phases, allowing the cost of securing migration state to be measured independently of the underlying Kubernetes security infrastructure.


% Network slicing allows logical networks to coexist on shared infrastructure \cite{sajjad2020interslice,etsi_ts122261_v16}, yet a significant implementation gap exists between theoretical mobility studies and realistic testbeds. In existing open-source stacks like OAI \cite{afolabi2018towards,kaltenberger2020openairinterface} and the Mosaic5G ecosystem \cite{mozaic5g}, moving a \ac{UE} between slices typically triggers a full \ac{NAS} re-registration. This involves identity exchanges and security re-negotiations as defined in the \ac{3GPP} \ac{SBA} \cite{3gpp.29.500,3gpp_slice_orchestra}. This migration incurs a switching latency averaging in the range of \textit{200–250 ms}. 

%Such delays cause service interruptions and signaling perturbations that are often abstracted away in these simulators and others like Network Simulator-3 (\textit{ns-3})~\cite{Henderson2008Network}.


%Orchra addresses these limitations by implementing a stateful inter-slice switching framework around OAI. Its design is anchored in three architectural components: \emph{state externalization}, \emph{control-plane interception}, and \emph{atomic user-plane re-anchoring}. Together, these components realize a migration path in which the UE context is temporarily externalized, the standard PDU Session Update is intercepted by a custom shim, and the target slice is brought into a ready state before the access-network switch is completed.
%To support the stateful migration of a UE from a source slice to a target slice without triggering standard 3GPP NAS re-registration loops or security renegotiations, \texttt{orchra} implements a modular signaling plane. This framework is explicitly structured into three distinct architectural phases that govern how context is decoupled, intercepted, and re-routed across the core network functions.


% \textbf{TODO:: Fix me and the numbers in this section} This setup allows us to compare three execution modes: full pod recreation, process-level restart, and Orchra-assisted migration. Table \ref{table:evaluation_metrics} illustrates the performance of network slice switching within our integral environment across these execution modes. %For the baseline setup, the results are categorized into two execution modes: pod-recreation and no pop-recreation (\textit{pkill}).
% In the pod recreation mode, the standard Kubernetes lifecycle triggers a complete container teardown, leading to on (\textbf{ToDo:: DESCRIBE ME IN TERMS OF THE CONFIDENCE INTERVALS }) a UE reattach delay of approximately \textit{2073.83 ms} due to the requirement for a cold-start radio synchronization. Instead of recreating the pod, in process-level restart mode, we simply restart the UE process within the existing container and this successfully minimizes the interruption to \textit{109.71 ms} (\textbf{TODO:: MAKE THE NUMBER 109 IN TERMS OF CIs and STD. DEVs}). \textbf{ToDo:: Figure 2 is not described AND ADD RESULTS DESCRIPTION FOR PATHLOSS AND JITTER}


%Finally, the orchestrator column demonstrates a significant reduction in latency by eliminating the need for Control Plane reconfigurations. Since the session migration is handled dynamically, the values for configuration patching, restart latency, and UE reattach delay are effectively zero, resulting in a average total switch time of \textit{38.267 ms}.

% The evaluation compares three execution modes for network slice switching: (i) full pod recreation using the standard Kubernetes lifecycle, (ii) process-level restart without recreating the running pod, and (iii) Orchra-assisted state migration. Table~\ref{table:evaluation_metrics} summarizes the switching performance across these modes, reporting the mean value, standard deviation, and 95\% confidence interval (CI) obtained from $N=200$ independent experiments. The end-to-end switching delay is the sum of the control-plane migration latency and the user-plane recovery latency, measured from migration trigger until the first packet is successfully forwarded through the destination UPF.

% The baseline pod recreation approach exhibits the highest interruption overhead. Since the complete container instance is terminated and recreated, the UE must undergo a full re-initialization procedure before resuming communication. This results in a total switching delay of $2099.17 \pm 33.29$~ms with a 95\% CI of $\pm6.52$~ms. The user-plane recovery component dominates this delay, with the first packet being delivered after $245.50 \pm 32.10$~ms ($\pm6.29$~ms CI). Furthermore, the disruption caused by the tear-down and recreation process negatively impacts data-plane stability, producing a packet loss rate of $12.45 \pm 1.82$\% ($\pm0.35$\% CI) and a transit jitter increase of $18.40 \pm 4.12$~ms ($\pm0.81$~ms CI).

% In contrast, the no-pod-recreation baseline performs substantially better by preserving the existing container environment and only restarting the UE process. This reduces the total switching delay to $161.26 \pm 18.11$~ms ($\pm3.55$~ms CI), representing a reduction of approximately 92.3\% compared with full pod recreation. The first packet recovery time decreases to $112.40 \pm 15.80$~ms ($\pm3.10$~ms CI). Although this approach avoids the overhead of container initialization, it still introduces measurable service degradation, resulting in a packet loss rate of $4.12 \pm 0.65$\% ($\pm0.12$\% CI) and a transit jitter delta of $9.15 \pm 2.04$~ms ($\pm0.40$~ms CI).

% Orchra-assisted migration further reduces the interruption by transferring the required execution state instead of recreating the network functions. The migration procedure consists of state export, state import, PFCP reconfiguration, and N2 completion phases, which require $15.24 \pm 2.11$~ms ($\pm0.41$~ms CI), $22.10 \pm 3.45$~ms ($\pm0.68$~ms CI), $8.15 \pm 1.02$~ms ($\pm0.20$~ms CI), and $2.86 \pm 1.84$~ms ($\pm1.73$~ms CI), respectively. Combining these control-plane operations with the user-plane recovery results in a total switching delay of only $49.72 \pm 10.67$~ms ($\pm3.46$~ms CI). The first packet delay is reduced to $1.86 \pm 1.57$~ms ($\pm1.73$~ms CI), demonstrating that preserving the session state significantly accelerates traffic resumption compared with both baseline approaches.

% The improvement achieved by Orchra is also reflected in the data-plane SLA metrics. Unlike pod recreation and process restart, which introduce packet losses of $12.45$\% and $4.12$\%, respectively, Orchra maintains continuous packet delivery with a measured packet loss rate of $0.00 \pm 0.00$\%. Additionally, Orchra reduces the transit jitter delta to $1.22 \pm 0.18$~ms ($\pm0.03$~ms CI), representing an improvement of approximately 93.4\% compared with pod recreation and 86.7\% compared with process-level restart.

% Table~\ref{table:evaluation_metrics} compares three network slice switching strategies: full pod recreation, process-level restart without pod recreation, and Orchra-assisted state migration. Results are reported as mean $\pm$ standard deviation with 95\% confidence intervals (CI) over $N=200$ independent experiments.

% The pod recreation baseline introduces the largest interruption due to complete container teardown and reinitialization. It results in a total switching delay of $2099.17 \pm 33.29$~ms ($\pm6.52$~ms CI), with a first packet delay of $245.50 \pm 32.10$~ms ($\pm6.29$~ms CI). This disruption also degrades data-plane performance, causing $12.45 \pm 1.82$\% packet loss ($\pm0.35$\% CI) and a transit jitter delta of $18.40 \pm 4.12$~ms ($\pm0.81$~ms CI).

% The no-pod-recreation baseline reduces the interruption by preserving the container environment and restarting only the UE process. This decreases the switching delay to $161.26 \pm 18.11$~ms ($\pm3.55$~ms CI) and the first packet delay to $112.40 \pm 15.80$~ms ($\pm3.10$~ms CI). However, process restart still introduces service degradation, resulting in $4.12 \pm 0.65$\% packet loss ($\pm0.12$\% CI) and $9.15 \pm 2.04$~ms jitter increase ($\pm0.40$~ms CI).

% Orchra-assisted migration avoids full reinitialization by transferring and restoring execution state. The migration overhead consists of state export ($15.24 \pm 2.11$~ms, $\pm0.41$~ms CI), state import ($22.10 \pm 3.45$~ms, $\pm0.68$~ms CI), PFCP reconfiguration ($8.15 \pm 1.02$~ms, $\pm0.20$~ms CI), and N2 completion ($2.86 \pm 1.84$~ms, $\pm1.73$~ms CI). Overall, Orchra achieves a switching delay of $49.72 \pm 10.67$~ms ($\pm3.46$~ms CI) and reduces first packet recovery to $1.86 \pm 1.57$~ms ($\pm1.73$~ms CI). It also maintains SLA-level performance with zero packet loss and only $1.22 \pm 0.18$~ms jitter variation ($\pm0.03$~ms CI).

%The security microbenchmark shows that AES-GCM protection introduces minimal overhead. Encryption increases write latency from $0.40 \pm 0.04$~ms to $0.95 \pm 0.08$~ms, while decryption increases read latency from $0.30 \pm 0.03$~ms to $0.75 \pm 0.06$~ms, resulting in a total cryptographic penalty of only $1.00 \pm 0.11$~ms ($\pm0.02$~ms CI).

% \begin{table*}[t]
%     \centering
%     \caption{Evaluation metrics for Orchra-assisted slice migration. Performance metrics are reported as mean $\pm$ standard deviation together with the 95\% confidence interval over $N=100$ independent experimental runs.}
%     \label{table:evaluation_metrics}
%     \rowcolors{3}{LightGray}{white}
%     \footnotesize
%     \begin{tabularx}{\textwidth}{@{}lYYY@{}}
%     \toprule
%     \textbf{Metric Component} & \textbf{Baseline: Pod Recreate} & \textbf{Baseline: No Pod Recreate} & \textbf{Orchra: State Migration} \\
%     \midrule
%         \textbf{Control Plane Performance} & & & \\
%         Export time ($t_{\mathrm{export}}$) [ms]       & -- & -- & $15.24 \pm 2.11$ [0.41] \\
%         Import time ($t_{\mathrm{import}}$) [ms]       & -- & -- & $22.10 \pm 3.45$ [0.68] \\
%         PFCP reconfiguration ($t_{\mathrm{pfcp}}$) [ms] & -- & -- & $8.15 \pm 1.02$ [0.20] \\
%         N2 completion ($t_{\mathrm{CP}}$) [ms]          & -- & -- & $2.86 \pm 1.84$ [1.73] \\
%     \midrule
%         \textbf{User Plane Performance} & & & \\
%         First packet delay ($t_{\mathrm{UP}}$) [ms]    & $245.50 \pm 32.10$ [6.29] & $112.40 \pm 15.80$ [3.10] & $1.86 \pm 1.57$ [1.73] \\
%         Total switching delay [ms]                    & $2099.17 \pm 33.29$ [6.52] & $161.26 \pm 18.11$ [3.55] & $49.72 \pm 10.67$ [3.46] \\
%     \midrule
%         \textbf{Data Plane Quality (SLA)} & & & \\
%         Packet Loss Rate [\%]                         & $12.45 \pm 1.82$ [0.35]   & $4.12 \pm 0.65$ [0.12]    & $\mathbf{0.00 \pm 0.00}$ \textbf{[0.00]} \\
%         Transit Jitter Delta ($\Delta J$) [ms]        & $18.40 \pm 4.12$ [0.81]   & $9.15 \pm 2.04$ [0.40]    & $\mathbf{1.22 \pm 0.18}$ \textbf{[0.03]} \\
%     \midrule
%         \textbf{State Micro-benchmarks (Security)} & & & \\
%         Write Path (Plaintext) [ms]                   & -- & -- & $0.40 \pm 0.04$ [0.01] \\
%         Write Path (AES-GCM Encrypted) [ms]           & -- & -- & $0.95 \pm 0.08$ [0.02] \\
%         Read Path (Plaintext) [ms]                    & -- & -- & $0.30 \pm 0.03$ [0.01] \\
%         Read Path (AES-GCM Decrypted) [ms]            & -- & -- & $0.75 \pm 0.06$ [0.01] \\
%         \rowcolor{LightPink} Net Cryptographic Penalty [ms] & -- & -- & $\mathbf{+1.00 \pm 0.11}$ \textbf{[0.02]} \\
%     \bottomrule
%     \end{tabularx}
% \end{table*}


%\textbf{FIX ME: THE NUMBERS AND DESCRIPTION OF RESULTS + FIGURE}

%The plaintext baseline achieves a highly deterministic profile with a mean reconfiguration latency of $38.27$ $ms$. When the Fernet encryption interceptor is activated, the structural encapsulation, serialization, and cryptographic signing loops scale the processing time down to the microsecond level per operation. This manifests as a minor, predictable parallel rightward shift across the entire distribution curve, adding an average computational overhead of approximately $1.24$ \textit{ms} [insert your actual delta here]. This empirical delta proves that implementing authenticated message-layer security over shared Redis infrastructure introduces a negligible latency penalty, preserving the deterministic sub-second profile required by ultra-reliable low-latency communication (URLLC) slices while completely neutralizing state-exfiltration vectors.

% Beyond the infrastructure-level protections provided by Kubernetes, Orchra secures externally stored session state through application-layer encryption. Before a migration context is written to Redis, the serialized PDU session state is encrypted using the Fernet authenticated encryption scheme, which combines \ac{AES}-128 in \ac{CBC} mode for confidentiality with \ac{HMAC}-\ac{SHA256} for integrity verification. Upon retrieval, the encrypted payload is authenticated, decrypted, and reconstructed into the native runtime structures required by the target SMF.

% This cryptographic processing is isolated within the storage access layer, allowing the evaluation to directly quantify the additional latency introduced by encryption and decryption during state externalization. Specifically, we measure the processing overhead added to the state export ($t_{\mathrm{export}}$) and import ($t_{\mathrm{import}}$) stages relative to plaintext state migration.

% The evaluation distinguishes between \emph{control-plane reconfiguration latency} and \emph{user-plane transition delay}. This distinction is necessary because Orchra eliminates the repeated NAS registration procedures associated with conventional slice switching while still requiring limited convergence for PFCP and N2 updates. The following timestamps are recorded throughout each migration:
% \begin{itemize}
%     \item $t_{\mathrm{trigger}}$: migration request issued by the orchestrator;
%     \item $t_{\mathrm{export}}$: source SMF completes session state export;
%     \item $t_{\mathrm{import}}$: destination SMF completes state restoration;
%     \item $t_{\mathrm{pfcp}}$: UPF acknowledges PFCP session modification;
%     \item $t_{\mathrm{n2}}$: AMF completes the N2 tunnel update;
%     \item $t_{\mathrm{first\_pkt}}$: first packet observed on the new GTP-U tunnel.
% \end{itemize}
% The individual state externalization delays are computed as
% \begin{equation}
%     \small
%     \begin{aligned}
%         \Delta t_{\mathrm{export}}
%         &=
%         t_{\mathrm{export}}
%         -
%         t_{\mathrm{trigger}}, \\
%         \Delta t_{\mathrm{import}}
%         &=
%         t_{\mathrm{import}}
%         -
%         t_{\mathrm{export}}.
%     \end{aligned}
% \end{equation}
% The end-to-end migration metrics are then defined as
% \begin{equation}
%     \small
%     \begin{aligned}
%         t_{\mathrm{CP}}
%         &=
%         t_{\mathrm{n2}}
%         -
%         t_{\mathrm{trigger}}, \\
%         t_{\mathrm{UP}}
%         &=
%         t_{\mathrm{first\_pkt}}
%         -
%         t_{\mathrm{trigger}}.
%     \end{aligned}
% \end{equation}
% \textit{Here, $t_{\mathrm{CP}}$ represents the control-plane reconfiguration latency, while $t_{\mathrm{UP}}$ denotes the user-plane transition delay experienced during migration.}

% \noindent For each metric, results are collected over $N=200$ migration runs and summarized using the mean, standard deviation, and 95\% confidence interval.

% The evaluation distinguishes between \emph{control-plane reconfiguration latency} and \emph{user-plane transition delay}. This distinction is necessary because Orchra eliminates the repeated NAS registration procedures associated with conventional slice switching while still requiring limited convergence for PFCP and N2 updates. The following timestamps are recorded throughout each migration:
% \begin{itemize}
%     \item $t_{\mathrm{trigger}}$: migration request issued by the orchestrator;
%     \item $t_{\mathrm{export}}$: source SMF completes session state export;
%     \item $t_{\mathrm{import}}$: destination SMF completes state restoration;
%     \item $t_{\mathrm{pfcp}}$: UPF acknowledges PFCP session modification;
%     \item $t_{\mathrm{n2}}$: AMF completes the N2 tunnel update;
%     \item $t_{\mathrm{first\_pkt}}$: first packet observed on the new GTP-U tunnel.
% \end{itemize}
% The state externalization delays are computed as
% \begin{equation}
%     \small
%     \begin{aligned}
%         t_{\mathrm{export}}
%         &=
%         t_{\mathrm{export}}
%         -
%         t_{\mathrm{trigger}}, \\
%         t_{\mathrm{import}}
%         &=
%         t_{\mathrm{import}}
%         -
%         t_{\mathrm{export}}.
%     \end{aligned}
% \end{equation}
% The end-to-end migration metrics are then defined as
% \begin{equation}
%     \small
%     \begin{aligned}
%         t_{\mathrm{CP}}
%         &=
%         t_{\mathrm{n2}}
%         -
%         t_{\mathrm{trigger}}, \\
%         t_{\mathrm{UP}}
%         &=
%         t_{\mathrm{first\_pkt}}
%         -
%         t_{\mathrm{trigger}}.
%     \end{aligned}
% \end{equation}
% \textit{Here, $t_{\mathrm{CP}}$ represents the control-plane reconfiguration latency, while $t_{\mathrm{UP}}$ denotes the user-plane transition delay experienced during migration.}

% \noindent For each metric, results are collected over $N=100$ migration runs and summarized using the mean, standard deviation, and 95\% confidence interval.

%This work addresses this gap through a stateful orchestration framework that preserves UE session context while enabling low-latency slice migration.

% Network slicing enables multiple logical networks to coexist over a common physical infrastructure, allowing slices to be tailored to heterogeneous service requirements such as \ac{eMBB}, \ac{URLLC}, and \ac{mMTC}~\cite{etsi_ts122261_v16,sajjad2020interslice}. Although the 3GPP architecture defines mechanisms for slice selection and lifecycle management, it does not specify a native procedure for seamless migration of an active User Equipment (UE) session between slices while preserving control- and user-plane state~\cite{3gpp.29.500,3gpp_slice_orchestra}. Consequently, most experimental platforms—including OAI and the Mosaic5G ecosystem—implement inter-slice switching by treating a change in the serving \ac{S-NSSAI} as a new registration procedure rather than as a state transfer~\cite{afolabi2018towards,kaltenberger2020openairinterface,mozaic5g}.

% As demonstrated by~\cite{Sajjad}, the lack of standardized session continuation mechanisms in the standard 3GPP Service-based Architecture forces a complete PDU session teardown and re-establishment, which can cause service disruption latencies to stretch significantly beyond these localized baselines when accounting for multi-hop core network signaling.
% Procedural standards suggest that, migrating a UE between slices triggers a complete NAS re-registration, including identity verification, authentication, security context establishment, and reconstruction of the PDU session~\cite{3gpp_slice_orchestra}. 
% These control-plane procedure introduces switching latencies ranging between $\mathrm{200-250\,ms}$ in our OAI/Mosaic5G testbed (Section~\ref{sec:evaluation})
% to introduce interruptions in user-plane forwarding and non-negligible transient packet losses. Such disruption is acceptable for infrequent mobility events but becomes a significant limitation for dynamic slice adaptation driven by Service Level Agreement (SLA) enforcement, Multi-access Edge Computing (MEC) offloading, or closed-loop \ac{RAN} optimization~\cite{Mohammedali}.

% A second limitation is the absence of a coordinated mechanism for transferring UE context across network functions. Existing open-source implementations execute migration as a sequence of loosely coupled operations across the \ac{AMF}, \ac{SMF}, and \ac{UPF}, without transactional guarantees or a shared state repository~\cite{mozaic5g}. As a result, failures or timing inconsistencies during migration can leave the control and user planes temporarily unsynchronized, producing incomplete session recovery or requiring the UE to repeat the registration procedure~\cite{sakic2020decoupling}. These shortcomings motivate the need for a state-persistent migration framework capable of preserving UE context while performing atomic control- and user-plane reconfiguration.

% Cross-border roaming further amplifies this implementation gap by introducing inter-\ac{PLMN} signalling, security, and policy coordination that are absent in single-domain deployments~\cite{Gallego}.
% For example, conventional Home-Routed Roaming has been reported to introduce service interruption approaching two minutes in connected mobility scenarios, motivating optimized 5G Standalone roaming procedures capable of reducing interruption to the order of hundreds of milliseconds \cite{kousaridas20215g,Marquez_etal}.
% When a UE moves from an \ac{H-PLMN} to a \ac{V-PLMN}, slice continuity becomes difficult because the visited network may not support the same S-NSSAI mapping, policy rules, or edge placement as the home network~\cite{afolabi2018network}. In practice, this often forces a full re-authentication and re-establishment of the session, introducing additional signaling delay and disrupting latency-sensitive services~\cite{saad2021slice}. The situation is even more constrained for ultra-low-latency applications, where home-routed roaming adds costly (hair-pinning - find me an alternative phrase) through the H-PLMN, while local breakout reduces latency but weakens home control over charging, security, and slice policy~\cite{roaming_arch}. These limitations show that preserving slice semantics across administrative domains is not just a mobility problem, but also a control-plane and service-continuity problem~\cite{taleb2019cross}. Emerging mechanisms such as slice roaming agreements, \ac{SEPP}-protected interconnects, and federated edge clouds point toward a solution, but a practical open-source testbed for evaluating stateful inter-slice migration under realistic roaming-like conditions is still missing~\cite{p1sec2026sepp, Nguyen_etal}.
% The proposed orchestration mechanism therefore targets rapid slice migration while preserving session continuity consistent with the mobility procedures defined in the 5G System architecture~\cite{3gpp.23.501}.

% \subsection{Novelty and Contributions}
% To address the limitations in these existing testbeds, we implement a stateful migration mechanism that reduces the Round Trip Time (RTT) closer to 3GPP requirements. Our primary contributions are as follows:
% \begin{itemize}
%     \item \textbf{Stateful Context Injection:} We design a transient staging layer that externalizes and injects serialized UE states (NAS counters, security keys, and \ac{PDU} contexts) directly into target NFs (Network Functions). Unlike Mosaic5G, which relies on re-registration, our approach preserves the UE's session state across slice boundaries.
%     \item \textbf{Network-side state injection} (reduced Control Plane RTT): We introduce an orchestration shim within the SMF (Session Management Function) that executes PDU session migration entirely within the network infrastructure, requiring near-zero signaling round-trips with the UE. By bypassing high-latency 3GPP standard \ac{NRF} discovery and inter-NF negotiation in favor of a direct redis-to-\ac{PFCP} state injection path, the system eliminates packet loss via proactive context hydration and synchronized buffering. This architectural shift reduces control plane switching latency from the $112.40\,\mathrm{ms}$ and $245.50\,\mathrm{ms}$ standard baseline to approximately $40–60\,\mathrm{ms}$. 
%     \item \textbf{Open-Source Framework:} We provide a reproducible, open-source experimental platform, enabling the research community to evaluate the operational viability of low latency slice migrations in 5G-Advanced and 6G environments.
% \end{itemize}

% The Core Bottleneck ("Apply and Switch"): The graph reveals that the Apply and Switch phase is the single most expensive operation in the migration pipeline. This is indicated by the steepest upward slope on the line, showing that the delta (time elapsed) during this transition is significantly larger than any other step. Physically, this represents the delay of updating the UPF datapath rules and rerouting active traffic.
% The nearly flat or low-gradient line between Trigger and Snapshot Context reveals that serializing the UE context and fetching state is highly optimized and introduces negligible delay to the overall process.
% To lower overall migration latency, optimization efforts should not be spent on state snapshot serialization, but rather on parallelizing or streamlining the actual switchover signaling (Apply and Switch) on the user plane.

% The proposed framework employs a two-layer security architecture to protect externally stored session state during inter-slice migration. The first layer secures the Redis state repository using standard Kubernetes mechanisms, including namespace isolation, access control policies, and secret management. As these deployment-level protections introduce negligible runtime overhead, they are not considered in the performance evaluation.

% Beyond the infrastructure-level protections provided by Kubernetes, \textbf{Orchra} protects externally stored session state using application-layer authenticated encryption. Before state externalization, each serialized PDU session context is encrypted using the Fernet scheme, which combines Advanced Encryption Standard (AES-128) encryption in Cipher Block Chaining (CBC) mode with Hash-based Message Authentication Code (HMAC)-Secure Hash Algorithm 256 (SHA-256) authentication. Upon retrieval, the target SMF verifies, decrypts, and reconstructs the session context.

% Since encryption and decryption are performed for every migration, we isolate these operations to quantify their contribution to the state export ($t_{\mathrm{export}}$) and state import ($t_{\mathrm{import}}$) latency relative to plaintext state migration.

% The state migration mechanism introduces a limited security-related processing overhead due to encryption. The plaintext write and read operations require $0.40 \pm 0.04$~ms and $0.30 \pm 0.03$~ms, respectively, while AES-GCM encryption and decryption increase these operations to $0.95 \pm 0.08$~ms and $0.75 \pm 0.06$~ms. Overall, the cryptographic protection adds a net penalty of only $1.00 \pm 0.11$~ms ($\pm0.02$~ms CI), indicating that secure state transfer can be achieved with minimal impact on migration performance.

% The graph reveals a massive throughput degradation on Writes when shifting from "Plain" to "AES". This is because encrypting data on every write operation is computationally heavy, creating a severe bottleneck for state export during migration.
% Conversely, Reads experience a much smaller relative performance drop. This reveals that the decryption process or cache-reading path is significantly faster and less CPU-bound than the encryption path.
% The stark contrast between the Plain and AES bars reveals that if your migration orchestrator relies on real-time, high-frequency state updates, enabling full payload AES encryption will severely limit your write transaction rate.

% This paper presented Orchra, a stateful inter-slice migration framework for OAI, Mosaic5G, and FlexRIC environments. The prototype demonstrates that stateful-aware switching is feasible through UE state externalization, control-plane interception, and atomic user-plane re-anchoring, minimizing the disruption window while preserving session continuity. However, generalizing this framework requires addressing several open challenges.
% First, native procedures for UE-level context migration or seamless inter-slice handovers are currently absent from 3GPP and O-RAN specifications~\cite{3gpp28541, oran2023}. Standardizing this capability will require extending SBI, E2, O1, and A1 interfaces to support vendor-neutral migration across core and RAN domains. Second, maintaining cross-component state consistency (e.g., NAS security, PDU sessions, QoS flows, tunnels) across the AMF, SMF, UPF, and RAN necessitates robust transaction semantics. Future iterations should incorporate rollback support and compensating execution models, such as SAGA-style workflows, to prevent race conditions or partial updates~\cite{smith2023}.

% Third, scaling the framework to large UE populations requires optimizing signaling efficiency and control latency. Mitigating orchestration bottlenecks, oscillation, and redundant switching will require predictive migration policies and hysteresis mechanisms, particularly in dense MEC deployments~\cite{lee2024, liu2022}. Fourth, security and privacy are paramount; externalizing subscriber data to a staging layer like Redis introduces exposure risks. Future deployments must integrate end-to-end encryption, auditable transitions, and confidential computing to protect context data in transit and at rest. Finally, evaluating Orchra beyond laboratory constraints—by introducing multi-tenant interference, mobility-induced load variations, and heterogeneous transport constraints—is essential to confirm system stability and failure resilience at scale~\cite{zhao2025, wang2024}.

%Furthermore, to guarantee deterministic throughput and prevent communication stalls caused by complex transport handshakes, the deployment variables enforce a strict fallback to an \texttt{\ac{HTTP}/1.1} interaction profile across these intercepted endpoints. This compressed \textit{Redis-to-PFCP} path strips away signaling hops, allowing the target SMF to finalize internal control-plane context reconstruction in sub-millisecond timelines. %~\cite{KALTENBERGER2020107284}.

% Network slicing is a foundational capability of \ac{5G}-Advanced and 6G architectures, yet practical mechanisms for maintaining service continuity during runtime slice transitions remain underdeveloped. 
% Standard cloud-native architectures like Mosaic5G and \ac{OAI} do not natively support stateful session migration; forcing slice changes requires intensive Non-Access Stratum (NAS) re-registration or container redeployment, introducing severe user-plane switching latencies ranging between $112.40\,\mathrm{ms}$ and $245.50\,\mathrm{ms}$ in localized environments. 
% To bridge this gap, we present \textbf{Orchra}\protect\footnote{\protect\url{https://github.com/anthonyKiggundu/okra}}, an intelligent orchestrator for stateful, low-latency context transfer. % \ac{S-NSSAI}
% By externalizing critical user equipment (UE) state---including active Non-Access Stratum (NAS) counters, cryptographic security keys, and \ac{PDU} session profiles---into an optimized, transient staging layer, Orchra ensures seamless session continuity across slice boundaries. 

% Quantitative results reveal that while standard \ac{3GPP} procedures can suspend user-plane traffic for latencies ranges between $112.40\,\mathrm{ms}$ and $245.50\,\mathrm{ms}$, Orchra slashes these latencies to ranges of  $40–60\, \mathrm{ms}$. Micro-benchmarks show that robust \ac{AES-GCM} state encryption adds a negligible processing overhead penalty of just $+1.267 \pm 0.11\,\mathrm{ms}$. 
% These empirical findings establish a reproducible, high-performance standard for low-latency, state-preserving slice transitions in \ac{5G}-Advanced networks.

% The proposed framework employs a two-layer security architecture to protect externally stored session state during inter-slice migration. The first layer secures the Redis state repository using standard Kubernetes mechanisms, including namespace isolation, access control policies, and secret management. As these deployment-level protections introduce negligible runtime overhead, they are not considered in the performance evaluation.

% Beyond the infrastructure-level protections provided by Kubernetes, \textbf{Orchra} protects externally stored session state using application-layer authenticated encryption. 
% Under the baseline \textit{plaintext} migration path, the source SMF serializes the active PDU session context into a raw JSON payload and writes it directly to the Redis database via standard socket operations. 
% Conversely, under the \textit{secured} path, each serialized JSON context is processed before externalization using Advanced Encryption Standard in Galois/Counter Mode (AES-GCM) with key lengths up to \textit{256 bits}. 
% This AEAD (Authenticated Encryption with Associated Data) scheme secures both confidentiality and integrity in a single pass by incorporating a unique \textit{96-bit} cryptographic initialization vector (nonce) alongside optional Associated Data (AAD). 
% Upon retrieval, the target SMF verifies the authentication tag, decrypts the ciphertext payload, and reconstructs the active session context.

% \begin{equation}
%     \small
%     \begin{aligned}
%         \Delta t_{\mathrm{export}}
%         &=
%         t_{\mathrm{export}}
%         -
%         t_{\mathrm{trigger}},\\
%         \Delta t_{\mathrm{import}}
%         &=
%         t_{\mathrm{import}}
%         -
%         t_{\mathrm{export}},\\
%         \Delta t_{\mathrm{update}}
%         &=
%         t_{\mathrm{pfcp}}
%         -
%         t_{\mathrm{import}}.
%     \end{aligned}
% \end{equation}

% \begin{equation}
%     \small
%     \begin{aligned}
%         t_{\mathrm{CP}}
%         &=
%         t_{\mathrm{n2}}
%         -
%         t_{\mathrm{trigger}},\\
%         t_{\mathrm{UP}}
%         &=
%         t_{\mathrm{first\_pkt}}
%         -
%         t_{\mathrm{n2}},\\
%         t_{\mathrm{switch}}
%         &=
%         t_{\mathrm{first\_pkt}}
%         -
%         t_{\mathrm{trigger}}
%         =
%         t_{\mathrm{CP}}
%         +
%         t_{\mathrm{UP}}.
%     \end{aligned}
% \end{equation}

      % t_{\mathrm{switch}}
        % &=
        % t_{\mathrm{CP}}
        % +
        % t_{\mathrm{UP}}.

        %\textit{Here, $\Delta t_{\mathrm{update}}$ captures the Southbound user-plane path-update latency over the N4 interface, $t_{\mathrm{CP}}$ captures the total duration of the control-plane migration, $t_{\mathrm{UP}}$ measures the additional forwarding recovery required before the first packet is delivered through the destination UPF, and $t_{\mathrm{switch}}$ represents the total service interruption experienced during slice migration.}

        % Here, $t_{\mathrm{export}}$ denotes the time required to serialize and externalize the session state at the source SMF, $t_{\mathrm{import}}$ captures the time required to retrieve and restore the session state at the destination SMF, $t_{\mathrm{pfcp}}$ represents the PFCP session reconfiguration latency over the N4 interface, and $t_{\mathrm{n2}}$ measures the duration of the N2 signaling required to complete the control-plane update. The aggregate control-plane migration latency, $t_{\mathrm{CP}}$, is the sum of these four phases. The user-plane recovery latency, $t_{\mathrm{UP}}$, measures the additional time until the first packet is successfully received through the destination UPF after completion of the control-plane migration. Finally, $t_{\mathrm{switch}}$ represents the total end-to-end service interruption experienced during slice migration.

